Self-Regularized Prototypical Network for Few-Shot Semantic Segmentation

The deep CNNs in image semantic segmentation typically require a large number of densely-annotated images for training and have difficulties in generalizing to unseen object categories. Therefore, few-shot segmentation has been developed to perform segmentation with just a few annotated examples. In this work, we tackle the few-shot segmentation using a self-regularized prototypical network (SRPNet) based on prototype extraction for better utilization of the support information. The proposed SRPNet extracts class-specific prototype representations from support images and generates segmentation masks for query images by a distance metric - the fidelity. A direct yet effective prototype regularization on support set is proposed in SRPNet, in which the generated prototypes are evaluated and regularized on the support set itself. The extent to which the generated prototypes restore the support mask imposes an upper limit on performance. The performance on the query set should never exceed the upper limit no matter how complete the knowledge is generalized from support set to query set. With the specific prototype regularization, SRPNet fully exploits knowledge from the support and offers high-quality prototypes that are representative for each semantic class and meanwhile discriminative for different classes. The query performance is further improved by an iterative query inference (IQI) module that combines a set of regularized prototypes. Our proposed SRPNet achieves new state-of-art performance on 1-shot and 5-shot segmentation benchmarks.

==> LaTex/method.tex <==

\section{Method}

\subsection{Problem Description}
{Few-shot segmentation~\cite{OSLSM,PANet,tian2020pfenet} aims at segmenting objects based on the support information from just a few annotated training images. Each few-shot segmentation task $\mathcal{T}$ (also named as an episode $\mathcal{T}$) consists of a support set $S$ supplied with ground-truth masks and a query set $\mathcal{Q}$.} The support set $\mathcal{S}=\{I, M\}$ contains only a few image - mask pairs. The query set $Q$ contains $N_q$ image-mask pairs. {Specifically in a $C$-way $K$-shot segmentation task where there are $C$ classes and $K$ support samples for each of the $C$ classes, we denote the support set as $\mathcal{S}=\{(I_{c,k},M_{c,k})\}$, where $k\in\{1,\cdots,K\}$ and $c\in\{1,\cdots,C\}$, indicating that $K$ image-mask pairs per semantic class from the $C$ classes are included. For example, for the class $c$, where $c\in\{1,...,c,...,C\}$, there are $K$ image-mask pairs as support samples, \ie, $\{(I_{c,1},M_{c,1}),(I_{c,2},M_{c,2})...,(I_{c,K},M_{c,K})\}$. The semantic classes are consistent in the support set and the query set, \ie, the query images are segmented to the $C$ classes (and the background class) provided in the support set. The goal is summarized as, to generate a model that, when given a support set $S$, predicts the annotation masks for the query images $Q$.}

The overall classes are divided into two non-overlapping sets of classes $C_{seen}$ and $C_{unseen}$, used for training and testing respectively. The training set $D_{train}$ is constructed from images of classes $C_{seen}$ and the testing set $D_{test}$ is constructed from images of classes $C_{unseen}$. Both the training set $D_{train}$ and the testing set $D_{test}$ contains lots of episodes $\mathcal{T}$. {The training set $D_{train}$ is composed of all image-mask pairs that contain at least one pixel in the segmentation mask from training classes. The testing set is randomly sampled. The testing classes $C_{unseen}$ are different from the training classes $C_{seen}$.}
Notably, for images in $D_{train}$, annotations of $C_{unseen}$ objects are excluded from the $D_{train}$ by labeling them as background, while the images are included as long as there is an object from $C_{seen}$ present.
The features are embedded from images by initializing CNN with pre-trained weights. During training, the model gains knowledge from the support set and then applies the knowledge to segment the query set. As each episode contains different semantic classes, the model can be well generalized after training. After obtaining the segmentation model $L$ from the training set $D_{train}$, we evaluate its few-shot segmentation performance on the test set $D_{test}$.

\begin{figure*}[t]
\begin{center}
  \includegraphics[width =1\textwidth]{LaTeX/Fig/fig2_cnn_compressed.pdf}
\caption{Architecture overview of our training model {in a 1-way 1-shot example}. We embed the support and query images into deep features by ResNet-50 with shared weights. Features from multiple levels are up-sampled and concatenated to form the final feature map. The prototypes, {including foreground one in yellow and background one in purple, are generated by masked average pooling over the support features.} Both the support images and the query images are segmented by computing the pixel-wise similarity between the prototypes and feature maps. The support loss $\mathcal{L}_{sup}$ and query loss $\mathcal{L}_{que}$ are used for end-to-end training.}
\vspace{0.16cm}
\label{fig:2}
\end{center}
\end{figure*}

\subsection{Architecture Overview}
As opposed to the parametric way that fuses the support and query features to generate segmentation masks, we aim to learn an accurate and robust class-specifical prototype representation. The learned prototype is good enough to represent the corresponding class and can deal with different kinds of objects/images, which performs segmentation via non-parametric metric learning. The overall architecture of the proposed training model is shown in \figurename~\ref{fig:2}. During each episode, images from the support and query set are embedded indiscriminately into deep features by a shared backbone. The masked average pooling (MAP) is then applied over the support features to produce prototypes. MAP is also useful in filtering background noise. The query images are segmented by assigning the class with the most similar prototype to each pixel. A self-regularization is applied to the prototypes, by segmenting the support images using their own prototypes. This operation encourages the few-shot model to generate more accurate prototypes as a prior to improving the consistency between support and query set.

Following~\cite{CANet, tian2020pfenet}, we adopt ResNet-50~\cite{resnet} as the backbone network. 
Besides, prototypes generated by the high-level feature maps of support images are usually abstract. To retain more details, we adopt a pyramid structure, where feature maps at various levels of the backbone extractor are aggregated to provide sufficient global scenery representation.
A pyramid feature aggregation is applied to the convolutional blocks to generate feature maps at different semantic levels. As shown in \figurename~\ref{fig:2}, these pyramid features are up-sampled to the same size and their concatenations are processed by a $1\!\times\!1$ \texttt{Conv} to 512 channels.
No extra free parameters will be introduced then. We aim to optimize the above-mentioned backbone to learn a consistent embedding space and train the model end-to-end.

\subsection{Prototype Generation}
Our model learns representative and well-separated prototype representation, {a feature vector}, for each semantic class, including the background, based on the prototypical network. We produce the foreground objects and background prototypes by applying the support masks over the feature maps separately. Given a support set $S=\{(I_{c,k},M_{c,k})\}$, where $c$, $k$ indexes the class and the shot respectively, let $F_{c,k}$ be the support feature map from the backbone and corresponds to the image $I_{c,k}$, the prototype of class $c$ is computed by masked average pooling:
\begin{equation}
    p_c=\frac{1}{K}\sum_k\frac{\sum_{x,y}F_{c,k}^{(x,y)}\mathbbm{1}(M_{c,k}^{(x,y)}=c)}{\sum_{x,y}\mathbbm{1}(M_{c,k}^{(x,y)}=c)},
\end{equation}
where $(x,y)$ indexes the coordinate location of pixels and $\mathbbm{1}(*)$ is an indicator function, outputting $0$ if $*$ is false or 1 otherwise. Similarly, we compute the background prototype by
\begin{equation}
    p_{bg}=\frac{1}{CK}\sum_{c,k}\frac{\sum_{x,y}F_{c,k}^{(x,y)}\mathbbm{1}(M_{c,k}^{(x,y)}=bg)}{\sum_{x,y}\mathbbm{1}(M_{c,k}^{(x,y)}=bg)},
\end{equation}
where $bg$ represents background. These prototypes are optimized non-parametrically during the end-to-end training as described in the following two sections.

\begin{figure}[t]
\begin{center}
  \includegraphics[width = 0.8\textwidth]{LaTeX/Fig/fig3_1_compressed.pdf}
\vspace{0.2cm}
\caption{Iterative Query Inference~(IQI). Multiple iteratively optimized prototypes, instead of a single prototype, are used for query inference. Each optimized prototype is based on the previous prototype’s evaluation of the supporting images. The final segmentation mask is generated by fusing the predicted annotations of each prototype.}
\vspace{0.12cm}
\label{fig:3}
\end{center}
\end{figure}

\subsection{Non-Parametric Distance Fidelity}
\label{section:34}
Here, we describe how the segmentation is performed using these prototypes and introduce our non-parametric distance fidelity.
We first calculate the similarity between each generated prototype over semantic classes (including background) and the feature vector $F_q^{(x,y)}$ at each position $(x,y)$ in the query feature. The softmax function is applied over the similarities to produce a probability map $\hat{M}_q$. Formally, given a distance function $\mathcal{D}$, let $\mathcal{P}=\{p_1,...,p_C\}\cup\{p_{bg}\}$ denote the prototype collection of prototype $p_c$ for class $c$ and $p_{bg}$ for background. For each $p_j\in \mathcal{P}$ (where $j=1,...,C\!+\!1$) and the query feature map $F_q$ we have
\begin{equation}
    \hat{M}^{(x,y)}_{q;j}=\frac{e^{\alpha\mathcal{D}(F_q^{(x,y)},p_j)}}{\sum_{j}e^{\alpha\mathcal{D}(F_q^{(x,y)},p_j)}},
\end{equation}
where $\alpha$ is an amplification factor.
The predicted segmentation mask is derived by 
\begin{equation}
    \hat{M}_q^{(x,y)}=\mathop{\arg\max}_{j} \hat{M}_{q;j}^{(x,y)}.
\end{equation}
The commonly adopted distance metric $\mathcal{D}$ is cosine distance~\cite{oreshkin2018tadam, PANet} and squared Euclidean distance~\cite{snell2017prototypical}. Here we introduce another distance metric, fidelity, which is defined as the distance between the respective density matrices of query features and prototypes. The density matrix as mentioned is defined formally as the outer product of a coordinate vector and its conjugate transpose. For each $F^{(x,y)}_q$ from query features and $p_j\in\mathcal{P}$ that both are reshaped to $1_{height}\times 1_{width}\times N_{channel}$, we first normalize them respectively by:
\begin{equation}
\begin{aligned}
    p_j&=\frac{p_j}{\lVert p_j\rVert},\\
    F^{(x,y)}_q&=\frac{F^{(x,y)}_q}{\lVert F^{(x,y)}_q\rVert}.
\end{aligned}
\end{equation}
The fidelity is then computed by:
\begin{equation}
    \mathcal{D}(F^{(x,y)}_q,p_j)= F^{(x,y)}_q\cdot (p_j^T \cdot p_j)\cdot (F^{(x,y)}_q)^T,
\end{equation}
where $p_j^T$ and $(F^{(x,y)}_q)^T$ is the transpose of $p_j$ and $F^{(x,y)}_q$, respectively. Both fidelity and cosine similarity measures distance from the direction rather than absolute value. Cosine similarity has a symmetrical value space about the origin, where the negative part is meaningless in the image segmentation. Unlike cosine similarity, the fidelity distributes only between 0 and 1 and thereby has a more evident distinction for vectors with different directions. 

Learning proceeds by minimizing the negative log-probability 
\begin{equation}
    \mathcal{L}_{que}=-\frac{1}{N}\sum_{x,y}\sum_{p_j\in\mathcal{P}}\mathbbm{1}(M_q^{(x,y)}=j)log\hat{M}^{(x,y)}_{q;j},
\end{equation}
where $N$ is the total number of spatial pixels, and $M_q$ is the ground truth mask of the query image. 


\subsection{Self-Regularized Prototype (SRP)}

In most previous works, the training process is only driven by the loss between predicted masks and ground truth masks of query images. Attempts (\eg, prototype alignment~\cite{PANet}) were devoted to improving the generalization of knowledge from support images to query images, which encourages the consistency of mutual generalizability between support and query images. However, in addition to the prototype alignment, it is also worth verifying the quality of the prototypes generated by the support set, \ie, the extent to which these prototypes can restore the support masks. We consider the feature extraction a process worth exploring and optimizing since if the prototype obtained from non-parametric average pooling on the support features is not a good representative, there is no way it will get a good performance on the query set. In fact, we have observed in experiments that the generated prototype did not restore the support images well  - losing many details and sometimes even not consistent when using the same prediction method as for the query images (see \figurename~\ref{fig:1}). This requires supervision on the  prototype generation process from support features.

To address these issues, we propose a Self-Regularized Prototype (SRP) module that can not only evaluate but also improve the quality of prototypes by incorporating the loss between the prototype-restored support masks and the original support masks. 
In this module, we adopt a more direct and effective method, which is to apply the prototypes to the supporting features to form support score maps. 
When the score maps are applied to pixel-wise feature vectors of support images themselves, supporting masks will be generated. 
The additional loss of the prototype-restored support masks and ground truth support masks are used for regularizing the prototype generation reversely. The prototype generation is therefore encouraged to retain specific details and enhance the distinction between classes. Meanwhile, considering that the generalization on support images is undoubtedly the best, the evaluation of the generated prototypes on support images will impose an upper bound of segmentation. The performance on query set will never exceed this upper bound set regardless of generalization. The consistency and generality between support and query can also be reasonably quantified in this way.

The proposed SRP is illustrated in \figurename~\ref{fig:2}. The prototypes obtained from support set 
are employed to generate segmentation masks for not only query set but also support set, following the method explained in section~\ref{section:34}. For each $p_j\in \mathcal{P}$ and each position's feature in support set $F_s^{(x,y)}$, we have
\begin{equation}
    \hat{M}^{(x,y)}_{s;j}=\frac{e^{\alpha\mathcal{D}(F_s^{(x,y)},p_j)}}{\sum_j e^{\alpha\mathcal{D}(F_s^{(x,y)},p_j)}}.
\end{equation}
The predicted segmentation mask for support set is then given by 
\begin{equation}
    \hat{M}_s^{(x,y)}=\mathop{\arg\max}_{j} \hat{M}_{s;j}^{(x,y)}.
\end{equation}
Similarly the loss between support predictions and annotations
\begin{equation}
    \mathcal{L}_{sup}=-\frac{1}{N}\sum_{x,y}\sum_{j}\mathbbm{1}(M_s^{(x,y)}=j)log\hat{M}^{(x,y)}_{s;j}.
\end{equation}
The overall training loss is
\begin{equation}
    \mathcal{L}=w_s\mathcal{L}_{sup}+w_q\mathcal{L}_{que},
\end{equation}
where $w_s$ and $w_q$ are used to balance the contribution of support loss and query loss. By SRP, we provide a quantification of the goodness of the learned prototypes, and meanwhile impel the network to learn more accurate and comprehensive prototypes and to generate more consistent prototypes for support and query sets, offering better segmentation performance.


\subsection{Iterative Query Inference~(IQI)}
A single prototype, though fine-tuned by end-to-end training, is not sufficiently explicit to segment an object due to the limited details it can retain and the large variation in object appearance within the same category. Usually, the prediction merely indicates the rough position and shape of the objects. To solve this issue, we propose an iterative collection of prototypes in query inference to further enhance the representative and generalization of prototypes according to their evaluation on support set. It's not necessary to include iterative optimization of prototypes in the training, because few commonality is observed in the detailed expression among different objects. 
The structure of our Iterative Query Inference~(IQI) is shown in \figurename~\ref{fig:3}, in which the prototypes are collected iteratively by:
\begin{equation}
    p_{j;n} = p_{j;n-1}-\eta\partial\mathcal{L}_{sup}/\partial p_{j;n-1},
\end{equation}
where $\eta$ is the reference rate and $\partial\mathcal{L}_{sup}/\partial p_{j;n-1}$ is the gradients, $n\in\{1,\cdots,N\}$ and $N$ is the amount of collected prototypes. We fuse the predicted score maps $\{\hat{M}_{q;j}^n:n=1,\cdots,N\}$ to generate the final segmentation $\hat{M}_{q}$ by
\begin{equation}
    \hat{M}_{q}=\mathop{\arg\max}_{j} \sum_{n=1}^N\hat{M}_{q;j}^n\rho_n,
\end{equation}
where $\rho_n=IoU(\hat{M}_s,M_s)$ is the intersection-over-union metric of evaluating the support set.

Our few-shot segmentation model adopts prototype embedding. Predictions are performed on the computed feature maps, thereby requiring no extra passes through the network. In addition, the proposed regularization is only imposed on the support features, avoiding repeated interaction between the support and query set. The computational cost for regularization occurs only in training, leaving inference free. Once the feature maps are extracted, no extra learnable parameters is introduced and thus is less prone to over-fitting.
